Robust Spoken Language Understanding via Paraphrasing

Learning intents and slot labels from user utterances is a fundamental step in all spoken language understanding (SLU) and dialog systems. State-of-the-art neural network based methods, after deployment, often suffer from performance degradation on encountering paraphrased utterances, and out-of-vocabulary words, rarely observed in their training set. We address this challenging problem by introducing a novel paraphrasing based SLU model which can be integrated with any existing SLU model in order to improve their overall performance. We propose two new paraphrase generators using RNN and sequence-to-sequence based neural networks, which are suitable for our application. Our experiments on existing benchmark and in house datasets demonstrate the robustness of our models to rare and complex paraphrased utterances, even under adversarial test distributions.

==> related.tex <==
\section{Related Work} \label{sec:related}

% spoken language understanding 
In this section we discuss prior research most related to this paper. The spoken language understanding literature mainly aims at learning a semantic meaning representation of a given user query. For most applications such meaning is represented in terms of a domain, intent, and slot labels  \cite{McCallumFreiPere:00,HafTurWri:03,WangDengAce:05,YamDenYuWang:08}. A variety of algorithms have been developed using unsupervised \cite{TurHakHil:11,HecHak:12}, supervised \cite{RayRic:07}, active learning \cite{TurSchHak:03} approaches. More recently, end to end deep learning based methods have also been proposed \cite{XuSar:13,MesDauYaoDengHakHe:15,HakTurCelChenGao:16,LiuLane:16}.

% sequence to sequence models
Encoder--decoder based deep neural networks for sequence learning have received considerable attention in the recent past due to its success in a variety of NLP tasks such as machine translation \cite{ChoBart:14,SutVinLe:14seq2seq}, parsing \cite{VinLuk:15,JiaLia:16,DongLap:16}, automatic text generation \cite{RushChoWes:15}, image captioning \cite{KarFei:17}, paraphrasing \cite{PraHasLee:16}. Techniques which improve basic sequence-to-sequence models by incorporating more encoder side information during decoding have been proposed e.g. using attention \cite{BahChoBen:15}, neural checklists \cite{KidZetCho:16checklist}, pointer networks \cite{VinForJai:15pointer}.

% paraphrase generation attacking out of vocabulary words in NLU
The problem of tackling rare and out-of-vocabulary words has particularly received attention in the problems of naural machine translation and different solutions have been proposed \cite{LuoSutLeVinZar:15,LuoMan:16}. The task of learning new command words in intelligent personal agents have also been studied recently \cite{ThoZhaMooSto:15,AzaKrisMit:16}.

Our paper studies the problem of learning a variety of paraphrased queries and out-of-vocabulary words in neural spoken language understanding systems.


